DarkSide-20k: A 20 Tonne Two-Phase LAr TPC for Direct Dark Matter Detection at LNGS

Building on the successful experience in operating the DarkSide-50 detector, the DarkSide Collaboration is going to construct DarkSide-20k, a direct WIMP search detector using a two-phase Liquid Argon Time Projection Chamber (LArTPC) with an active (fiducial) mass of 23 t (20 t). The DarkSide-20k LArTPC will be deployed within a shield/veto with a spherical Liquid Scintillator Veto (LSV) inside a cylindrical Water Cherenkov Veto (WCV). Operation of DarkSide-50 demonstrated a major reduction in the dominant $^{39}$Ar background when using argon extracted from an underground source, before applying pulse shape analysis. Data from DarkSide-50, in combination with MC simulation and analytical modeling, shows that a rejection factor for discrimination between electron and nuclear recoils of $\gt3\times10^9$ is achievable. This, along with the use of the veto system, is the key to unlocking the path to large LArTPC detector masses, while maintaining an "instrumental background-free" experiment, an experiment in which less than 0.1 events (other than $\nu$-induced nuclear recoils) is expected to occur within the WIMP search region during the planned exposure. DarkSide-20k will have ultra-low backgrounds than can be measured in situ. This will give sensitivity to WIMP-nucleon cross sections of $1.2\times10^{-47}$ cm$^2$ ($1.1\times10^{-46}$ cm$^2$) for WIMPs of $1$ TeV$/c^2$ ($10$ TeV$/c^2$) mass, to be achieved during a 5 yr run producing an exposure of 100 t yr free from any instrumental background. DarkSide-20k could then extend its operation to a decade, increasing the exposure to 200 t yr, reaching a sensitivity of $7.4\times10^{-48}$ cm$^2$ ($6.9\times10^{-47}$ cm$^2$) for WIMPs of $1$ TeV$/c^2$ ($10$ TeV$/c^2$) mass.

==> ReD.tex <==
%---
\section{Nuclear Recoil Calibration with R\lowercase{e}D}
\label{sec:ReD}

Precise understanding of the scintillation and ionization signals produced by Ar nuclear recoils (NR) in \LAr\ will be necessary for the interpretation of data from \DSk.  Members of the \DS\ collaboration performed  the \SCENE\ experiment~\cite{Alexander:2013ke,Cao:2015ks} in~2013, providing information on the recoil energy and electric field dependence of these signals which was important in the analysis of \DSf~\cite{Agnes:2016fz}.  For \DSk, a set of groups from the \DS\ Collaboration plan to perform a dedicated set of experiments to obtain additional measurements needed to extend the range and improve the precision of the \SCENE\ results.

The plan is to expose a small \LArTPC\ to variable-energy neutron beams and to study single elastic neutron scatters from argon nuclei, as was done in \SCENE.  Improvements compared to \SCENE\ will include use of the Geiger-mode avalanche photodiode \TPC\ (\GAPTPC), a purpose-built small \LArTPC\ using \DSk\ photodetectors and having very high light yield for improved photoelectron statistics.  Neutron-generator and accelerator-produced beams will be used as needed to extend the recoil nucleus energy range from the \SCENERecoilsEnergyMax\ maximum of \SCENE\ up to about \ReDRecoilsEnergyMax.  Finally, the tantalizing possibility of a variation of the NR signals as a function of their directions relative to the applied drift (electric) field will be studied with a definitive high-precision and high statistics dataset.

Sensitivity to the direction of the nuclear recoils originating from \WIMP\ scatters would be a very highly desirable capability for a direct dark matter detection experiment.  It would provide a powerful signature (perhaps the only one) for identifying any observed signal with the galactic halo dark matter~\cite{Spergel:1988fg,Gondolo:2002fg}.  Detailed calculations have shown that in the standard isothermal halo model, just a few to several tens of events are required for a statistically significant directional signal~\cite{Morgan:2005hm}, depending on the angular resolution of the detection method.  Even structures beyond the isothermal halo, like galactic tidal streams, have been shown to give observable effects in detectors with very limited directional sensitivity~\cite{Freese:2005iy}   

Initial Recoil Directionality (\ReD) experiments will be carried out at Universit\`a degli Studi di Napoli ``Federico II'', using a $d-d$ neutron generator delivering monoenergetic neutrons of \DDNeutronEnergy.  Later the experiment will move to the INFN Laboratori Nazionali del Sud (\LNS) in Catania.  For \ReD, near-exclusive use of beam as well as dedicated target rooms  have been made available at Napoli and \LNS\ for long-term installation and running of the \ReD\ detector.  This mode of operation will enable lengthy runs with a stable proton/ion beam at the desired energy, see Sec.~\ref{sec:ReD-LNS}.  The inability to perform very long runs in a stable setup was another limitation of the \SCENE\ experiment, performed in user mode at the accelerator lab of Notre Dame University.

Fig.~\ref{fig:ReD-Sketch} shows a schematic drawing of the experiment.  \LArTPC\ signals from neutron elastic scattering nuclear recoils of energy \ReDRecoilsEnergyRange\ in \LAr\ will be recorded in the \LArTPC, in coincidence with signals from the scattered neutron interacting in neutron detectors placed at various scattering angles relative to the beam.  The coincidence kinematics allow the energy and direction of the nuclear recoils occurring in the \LAr\ target to be precisely known event-by-event, given the beam energy and the scattered neutron angle.  As demonstrated in \SCENE~\cite{Alexander:2013ke,Cao:2015ks}, the coincidence technique combined with time-of-flight and the \PSD\ capabilities of both the \LArTPC\ and the neutron detectors  can give a very clean selection of single-scatter neutron elastic events.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{./ReD-Sketch.pdf} 
\caption{Schematic drawing of the \ReD\ experimental setup.}
\label{fig:ReD-Sketch}
\end{figure*}

\SCENE\ produced a study of the response of nuclear recoils in \LAr\ as a function of drift field~\cite{Alexander:2013ke,Cao:2015ks},  demonstrating that electron-ion recombination and primary scintillation yield for nuclear recoil tracks in \LAr\ depend strongly on the applied drift field.  \SCENE\ also characterized the energy dependence of ionization by nuclear recoils and \grs, and performed an initial search for a dependence of the nuclear recoil response upon the direction between the drift field and the initial momentum of the recoil.  This  gave tantalizing hints of a possible directional signal above \SCENEDirectionalityThreshold\ in \LAr, but no statistically significant result.  Factors limiting the precision of \SCENE\ included the use of  cryogenic \DSfPMT\ \PMTs, whose inherent instability at LAr temperature was exacerbated by the high-rate environment of the accelerator target room and the high dynamic range of the primary scintillation vs. ionization signals.  This limited the beam intensity that could be tolerated, and hence the attainable statistics, as well as introducing a number of corrections from the several monitoring systems.

The \ReD\ detector itself is a new type of \LArTPC, the \GAPTPC, whose innovative design takes advantage of the availability of \SiPMs\ to increase the photoelectron yield and greatly improve the stability of the photosensor response.  The \ReD\ \GAPTPC\ will be instrumented with tiles of the new-generation \SiPMs\ currently being developed for the \DS\ Collaboration, which are discussed in Sec.~\ref{sec:PhotoElectronics}.  The design of the \GAPTPC\ maximizes the light collection efficiency, with \SiPMs\ placed on the lateral surface of the detector as well as the top and bottom, see Sec.~\ref{sec:ReD-GAPTPC}.

The large-acceptance neutron spectrometer is designed to select and measure single-scatter neutron  elastic  events on argon (Sec.~\ref{sec:ReD-NeutronsSpectrometer}).  The spectrometer consists of an array of liquid scintillator neutron detectors on precision mounts which, combined with variable-angle neutron beams, allow the neutron-\TPC\ coincidences to select nuclear recoils at desired angles to the (perforce vertical) \GAPTPC\ drift field, including \num{0} and \SI{90}{\degree}.  A directional dependence would manifest itself as a difference in the scintillation and/or ionization response for nuclear recoils of the same energy but different track orientations, selected from data of a single run according to which neutron detector fired.

Directional effects on both scintillation light and ionization yield are expected in the recoil energy range relevant for dark matter searches, due to the phenomenon of columnar recombination in \LAr~\cite{Jaffe:1929gz,Jaffe:1913gs,Jaffe:1913cf,Swan:1965ha}.  Columnar recombination models suggest that the amount of ionization charge recombination (and therefore the  size of \STwo\ relative to \SOne) should, under some circumstances, vary with the angle between the field and the track direction.  When electrons are forced to drift through a column of ion-electron pairs produced by the ionizing track, the recombination probability is enhanced.  Larger effects are expected for tracks more energetic than the maximum measured with \SCENE.  Evidence for a subtle directional effect on $\alpha$-particle scintillation field-quenching  was seen long ago~\cite{Hitachi:1992gq}, but an effect useful for dark matter searches has not been found.

The \ReD\ experiment is also designed to provide a detailed characterization of the direction-averaged  nuclear recoils in \LAr\ in the presence of drift fields.  The optimized design of the \GAPTPC\ will minimize the probability of contamination from multiple neutron scatters inside the active volume.  The liquid scintillator neutron spectrometer will allow a large sample of nuclear recoil events to be collected in the energy region of interest for dark matter detection.  With a slight modification of the setup, electron recoils in \LAr\ will also be thoroughly studied, to help understand the response to electron recoil backgrounds.  Back-to-back \PositronAnnihilationGammaEnergy\ coincident \grs\ from a \ce{^22Na} positron source will provide a clean sample of events associated with a single Compton interaction in the argon detector, triggered on coincidences with a liquid scintillator behind the source.  A second liquid scintillator, shielded by a collimator, will be located at a known (variable) angle with respect to the line of travel of \grs, to select a precise electron recoil energy in \LAr.  By comparing the electron recoil energy with the nuclear recoil energy from the neutron beam measurements, one can map the ionization and scintillation efficiency as a function of the electric field and of the energy.

The success of the \ReD\ experiment could have a crucial impact on the broader program of the \DS\ Collaboration.  Aside from the added precision and range of detector response measurements, the discovery of sensitivity to the direction of recoils in liquid argon would revolutionize the field of dark matter direct searches and would provide a formidable asset for \DSk\ and \Argo.


%---
\subsection{The \ReD\ \GAPTPC}
\label{sec:ReD-GAPTPC}

The ReD experimental setup is designed to minimize all neutron interactions other than single scatters in the liquid argon.  This is achieved in two ways: by reducing as much as possible the material between the neutron beam and the \LAr, and with an innovative structure for the \LAr\ detector which minimizes the presence of inactive volumes.

The conceptual design of the \GAPTPC\ detector has been described in Ref.~\cite{Rossi:2016jg}.  It is conceived to achieve a very high light of \GAPTPCLightYield, an exceptional single photon resolution of \GAPTPCSPEResolution, and spatial resolution of \GAPTPCSpatialResolution\ in each of the two directions in the $x-y$ plane, which will considerably improve the multi-hit events rejection.

A first step towards the \GAPTPC\ was taken at Naples by building a prototype \LArTPC\ with \SiPM\ readout.  In the present configuration, the detector design closely follows that used in \SCENE.  The active volume is contained within a \GAPProtoActiveDiameter\ diameter, \GAPProtoActiveHeight\ tall, \PTFE\ support structure lined with Lumirror enhanced specular reflector and capped by fused silica windows.  The \LAr\ is viewed through the windows by two \SiPM\ \DSkTileAreaStd\ tiles.  The windows are coated with \ITO, allowing for the application of electric field, and copper field rings mounted on the \PTFE\ structure maintain field uniformity.  All internal surfaces of the detector are evaporation-coated with \TPB.  A hexagonal stainless steel mesh is fixed at the top of the active \LAr\ volume and electrically grounded to provide the drift field (between the bottom window and the mesh) and the extraction and amplification fields (between the mesh and the top window).

This detector will be used for the preliminary tests of the neutron beam line.  Once installed into the experimental hall and coupled with a few neutron detectors of the neutron spectrometer, a preliminary test of the whole experimental facility will be made, with the initial objective of reproducing the results of the \SCENE\ experiment.  

The \GAPTPC\ (see Fig.~\ref{fig:ReD-TPC}) will have a cylindrical size of about \GAPTPCActiveDiameter\ diameter and height.  A fused silica vessel defines the active volume, with the top and bottom windows \ITO\ coated to allow for the application of the electric field.  Near the top, a hexagonal mesh grid terminates the drift field and allows the higher extraction field to be applied between it and the anode.  The drift field is kept uniform along the drift coordinate by means of field shaping rings, deposited by thin coating the walls of the fused silica vessel with \ITO.  The \GAPTPC\ will not make use of any reflectors. Different size optical readout detector modules will be installed all around the fused silica cylinder to achieve $4\pi$ coverage.  

\begin{figure}[t!]
\centering{} 
\includegraphics[width=0.5\columnwidth]{./ReD-TPC.png}
\caption{A 3D rendering of the proposed \GAPTPC\ detector.}
\label{fig:ReD-TPC}
\end{figure}

A simple readout system based on CAEN~VT1730 14-bit 500 MS/s waveform digitizers is being setup for  
the \GAPTPC.  For the top array it is planned to individually read out each of the \SiPM\ dies in order to better study the \STwo\ signal distribution on the photosensors top plane, thereby enhancing the $x-y$ resolution.  The bottom plane, that does not take part in the $x-y$ reconstruction of the events, can be readout by a single channel or more, if required by signal to noise considerations.  The plan is to optimize the readout granularity of the lateral surface by Monte Carlo simulations.  The total number of signal output channels will be in the range 35-50.  Signal outputs will be fed to an external front-end amplifier and then to the waveform digitizer system.  The same readout will be used for the liquid scintillator channels of the neutron spectrometer, described below.  Digitized waveforms will be recorded based on a hardware trigger generated by a coincidence of channels above threshold.  In a later stage, a more sophisticated trigger will be deployed allowing more complex coincidence between the \LArTPC\ and the liquid scintillator counters.

\LArTPCs\ are usually housed within vacuum insulated (double walled) stainless steel cryostats, surrounded by a buffer region of inactive argon.  In this design, the main body of the TPC is a transparent fused silica vessel defining the active volume.  All photosensors and the ancillary equipment are placed outside the vessel so as to completely eliminate backgrounds due to the presence of a buffer of passive argon outside the \TPC.  The \GAPTPC\ will be housed in a single-walled stainless steel cryostat.  The cryostat will be equipped with thin windows for entry and exit of the neutron beam, if the simulation studies which are underway will suggest so.  An indium-sealed top flange will seal the cryostat and will mount a series of additional smaller flanges and feedthroughs needed for vacuum, \LAr\ fill, signal and HV cables, optical fibers for calibration laser signals, pressure, temperature and level monitors, safety valves, etc.  A Cryomech PT90 pulse-tube provides the cooling power through a heater block down to a condenser and cooling rods to the sensors.

Commercial argon gas will be initially passed through a commercial getter in order to remove impurities (mainly oxygen, nitrogen and water) from both the input gas and the detector components.  The system will be equipped with a gas recirculation loop, including the possibility of injection of a gaseous \ce{^{83m}Kr} source.

An additional innovative liquid recirculation system is available in Naples.  The system consists of a mechanical bellows pump coupled with a Trigon filter placed in the vacuum jacket of the cryostat.  Commercial pumps for cryogenic liquid make use of lubricants that can spoil the \LAr\ purity during the recirculation, and usually run only at a fixed speed.  The custom-designed Naples mechanical pump uses no lubricant, and furthermore cannot induce any electronic noise on the detector front end.  It also has the flexibility to adjust the recirculation speed as needed for the experiment, and finally it is much cheaper than commercial alternatives.

The \GAPTPC\ cryogenics will be equipped with an automated slow control system.  The \LAr\ filling and emptying procedure, the LAr and the gas recirculation and the exhaust safety  line will be automated by means of pneumatic valves controlled by the slow control system.  This allows parameters of the system to be changed while the neutron beam is on, without entering in the experimental hall.  It is also very beneficial in case of, {\it e.g.}, a power failure of the cryocooler, since it allows an automatic quick intervention on the cryogenic system to put the system in a safe and steady condition if needed.

The slow control system will be LabView based, allowing the necessary flexibility without excessive software effort.  The software architecture will be a state machine able to read, write, and display values using a graphical user interface.  The slow controls will interface with the DAQ system.  In particular, before each run there will be a complete check of the parameters and the status of the system will be logged in a file read by the DAQ.


%---
\subsection{Neutron Beam at \LNS}
\label{sec:ReD-LNS}

A suitable neutron beam can be produced by the accelerator facilities of the INFN \LNS, using any one of a variety of production reactions.  Floor space is available to install the \ReD\ \LArTPC\  at about \SI{1}{\meter} from the interaction point, with all ancillary services and the neutron spectrometer.  The \RedLNSDistanceDedicatedLine\ beam line at the \LNS\ Tandem accelerator has been dedicated for this purpose by the \LNS\ Scientific Committee.  This will allow stable long-term operation of  the experiment and to accumulate statistics 
over many runs.

The \LNS\ Tandem accelerator has a maximum terminal voltage of \RedNaplesVoltage\ and good reliability.  It has been recently upgraded, replacing the original charging belt by a pelletron system, with excellent voltage stability verified both at low and high terminal voltages.  Many isotopes can be accelerated by the Tandem, with the exception of noble gases.  The maximum current ranges from \RedNaplesCurrent\ typically.

As the Tandem cannot be operated in pulsed mode, the energy of the produced neutron must be reconstructed event by event using kinematics, detecting the angle and the energy of the charged particle produced along with the neutron in the reaction.  The detection of the charged particle will provide the start for a time-of-flight measurement of the scattered neutron.  The coincidence between the charged particle detector and the \LArTPC\ will be recorded in the \DAQ, contributing an additional method for background reduction.  Among the variety of possible reactions for neutron production, the following set is considered:
\begin{inparaenum}
\item $p$(\ce{^7Li},\ce{^7Be})$n$;
\item $d$($d$,\ce{^3He})$n$;
\item \ce{^197Au}($d$,$np$)\ce{^197Au}.
\end{inparaenum}

Preliminary measurements will be performed using a simple neutron detector, in order to chose the most favorable reaction for the \ReD\ purpose and to study the room background, to minimize parasitic interactions which would spoil the global performance.  For this purpose, the \RedLNSDistanceDedicatedLine\ beam line must be completely refurbished, to optimize the layout and to accommodate a new beam dump and the \LArTPC.  Moreover, a new custom-made scattering chamber is being built to host the production targets and the Si detectors used for charged particle detection, featuring thinner walls and an exit window in the outgoing neutron direction, to minimize the neutron interactions.


%---
\subsection{\lowercase{n}T\lowercase{o}F Spectrometer}
\label{sec:ReD-NeutronsSpectrometer}

To measure the scattered neutrons, the \ReD\ experiment will use an array of liquid scintillator neutron detectors that can measure the neutron scattering angles and the neutron time-of-flight (\TOF).  In this way, for  monochromatic neutrons single-scattered from \LAr, the kinematics is fully determined and the \ce{^40Ar} recoil energy and direction can be reconstructed, and background from direct neutrons coming from the production target or random coincidences of neutrons with signals in the \TPC\ can be suppressed.  The proposed  neutron spectrometer is based on \RedLNSNeutronSpectrometerDetectorsPMTsDiameter\ liquid scintillator counters from \RedLNSNeutronSpectrometerDetectorsManufacturer, using \RedLNSNeutronSpectrometerDetectorsScintillatorType\ liquid scintillator coupled to \RedLNSNeutronSpectrometerDetectorsPMTsType\ \PMTs.  These tubes are fast enough to provide accurate \TOF\ with a precision of around \RedLNSNeutronSpectrometerDetectorsPMTsTimeResolution.  These detectors can provide separation between neutron-induced and other signals, by using of pulse shape discrimination, from \RedLNSNeutronSpectrometerDetectorsPSD.  The plan is to use \RedLNSNeutronSpectrometerDetectorsNumber\ of such counters in the array, allowing one to record data for different recoil kinematics simultaneously.  The geometry is still to be finalized.  One scheme foresees the construction of a lightweight mechanical structure where counters can be placed at different angles on support guides held at constant radius from the \LArTPC\ center.  The support structure would allow simultaneous detection of  scattered neutrons corresponding to a given recoil energy but producing recoil argon atoms at different angles with respect to the electric field direction.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\columnwidth]{./ReD-NeutronSpectrometerFront.pdf}
\caption{Proposed ReD neutron spectrometer geometry and support structure.}
\label{fig:ReD-NeutronSpectrometerFront}
\end{figure}

